The Synchronization Power of Auditable Registers

Auditability allows to track all the read operations performed on a register. It abstracts the need of data owners to control access to their data, tracking who read which information. This work considers possible formalizations of auditing and their ramification for the possibility of providing it. The natural definition is to require a linearization of all write, read and audit operations together (atomic auditing). The paper shows that atomic auditing is a powerful tool, as it can be used to solve consensus. The number of processes that can solve consensus using atomic audit depends on the number of processes that can read or audit the register. If there is a single reader or a single auditor (the writer), then consensus can be solved among two processes. If multiple readers and auditors are possible, then consensus can be solved among the same number of processes. This means that strong synchronization primitives are needed to support atomic auditing. We give implementations of atomic audit when there are either multiple readers or multiple auditors (but not both) using primitives with consensus number 2 (swap and fetch&add). When there are multiple readers and multiple auditors, the implementation uses compare&swap. These findings motivate a weaker definition, in which audit operations are not linearized together with the write and read operations (regular auditing). We prove that regular auditing can be implemented from ordinary reads and writes on atomic registers.

==> Packages.tex <==
% \usepackage{algorithmic} 
\usepackage[ruled]{algorithm}
\usepackage[noend]{algpseudocode} %Not accepted..

\usepackage{xcolor}

\usepackage{tabularx}


%%%%%%%%%%%%%% Unecessary package? %%%%%%%%%%
% \usepackage{textcomp}
% \usepackage{cite}
% \usepackage{ulem}


%%%%%%%% ALREADY INCLUDE %%%%%%%%%%%
% \usepackage{enumitem}

% \usepackage[colorlinks=true, allcolors=blue]{hyperref} %?
% \usepackage{graphicx}
% \usepackage{amsmath,amsfonts,amssymb}
% \usepackage{tabularx}





%%%%% Old %%%%%

% \PassOptionsToPackage{unicode}{hyperref}
% \PassOptionsToPackage{naturalnames}{hyperref}
% \pdfstringdefDisableCommands{%
%   \def\\{}%
%   \def\texttt#1{<#1>}%
% }

% \usepackage{makecell} %????
% \usepackage{tikz} %??????

==> algorithms/AtomicAuditableRegister/SWMRMA.tex <==


% { % \footnotesize
% \begin{algorithmic}[1]
% \Statex \textbf{Shared Variables:}
% \Statex $\mathit{R}$ accessed with $\mathit{read}$, $\mathit{fetch\&add}$, $\mathit{compare\&swap}$,
% % Object shared between the $n$ processes that can be accessed through the following operations: \textit{read}, $\mathit{compare\&swap}$, $\mathit{fetch\&add}$. 
% initially $v_0*2^n$.
% \Statex $\mathit{R_{index}}$ accessed with $\mathit{read}$, $\mathit{write}$,
% % Register shared between the writer and the auditors that can be access through $\mathit{write}$ operation by the writer and $\mathit{read}$ operation by the auditors. 
% initially $0$.
% \Statex  $\mathit{pairs[\,]}$ An unbounded array of $\mathit{read}$/$\mathit{write}$ registers, initially all registers $\perp$. %Each register accessed with $\mathit{read}$ and $\mathit{write}$ operation. Initially all registers $\perp$.
% % An unbounded array of objects, shared between the $n$ processes. All the processes can access it through \textit{read} operation and the writer can additionally access it through a \textit{write} operation. Initially all registers $\perp$.

% \Statex 
% \Statex \textbf{Local Variables:} \Comment{{\bf Pseudo code for reader $p_i$, $i\in[0,n-1]$}}
% \Statex $\mathit{read\_result}$ initially $\perp$ \Comment{the last value read}
% \Statex $\mathit{val}$ initially $\perp$ \Comment{the content of the register} 

% \START[Read()] 
%     \State{$\mathit{val} \gets \mathit{R.read()}$}
%     \label{line:swmrma:read}
%     \START[if]{ $(\mathit{val} \pmod{ 2^{(i+1)}})/2^{i} = 0$}
%     \label{line:swmrma:readCondition}
%     \State{$\mathit{read\_result},  \gets \mathit{R.fetch\&add}(2^i)$}
%     \label{line:swmrma:readFetch}
%     \EndPhase
%     \State{\textbf{return} $\mathit{read\_result}/2^n$}
%     \label{line:swmrma:readReturn}
% \EndPhase

% \Statex 
% \Statex \textbf{Local Variables:} \Comment{{\bf Pseudo code for auditor $p_i$, $i\in[0,n-1]$}}
% \Statex $\mathit{val}$, initially $\perp$ \Comment{the content of the register} 
% \Statex $\mathit{audit\_result}$, initially $\emptyset$ \Comment{set of couples (process, value)} 
% \Statex $\mathit{audit\_index}$, initially $0$ \Comment{index of the last updated couple in $pairs$} 
% \Statex $\mathit{last\_index}$, initially $0$ \Comment{index used during the last audit operation} 

% \START[Audit()]
%     \State{$\mathit{val} \gets \mathit{R.read()}$}
%     \label{line:swmrma:auditRead}\State{$\mathit{audit\_index}, \gets \mathit{R_{index}.read()}$}
%     \label{line:swmrma:auditReadIndex}
%     \START[for]{ $\mathit{last\_index} \leq i < \mathit{audit\_index}$}
%         \State{$\mathit{audit\_result}.add(pairs[i].read())$}
%         \label{line:swmrma:auditAddAuditPairs}
%     \EndPhase
%     \State{$\mathit{last\_index} \gets \mathit{audit\_index}$}
%     \START[for] $0 \leq i < n$
%         \START[if] $(\mathit{val} \pmod{ 2^{i+1}})/2^{i} = 1$
%             \Comment{checks if $p_i$ read the last value written in S}
%             \label{line:swmrma:auditCondition}
%             \State{$\mathit{audit\_result}.add(p_i,\mathit{val}/2^{n})$}
%             \label{line:swmrma:auditAddAudit}
%         \EndPhase
%     \EndPhase  
        
%     \State{\textbf{return} $\mathit{audit\_result}$}      
% \EndPhase

% \Statex 
% \Statex \textbf{Local Variables:} \Comment{{\bf  pseudo code for writer $p_0$}}
% \Statex $\mathit{val}$, initially $v_0*2^n$ \Comment{the last value in the register}
% \Statex $\mathit{index}$, initially $0$ \Comment{index of the last couples in $pairs$ for audit} 
% \Statex $\mathit{set}$, initially $\emptyset$ \Comment{store the reads detected during the current write} 
% % \Statex $\mathit{new\_index}$ initially $0$ \Comment{the couple (process, value) of all the read operations} 

% \START[Write($v$)]
%     \START[while]{$(\mathit{R.compare\&swap}(\mathit{val},v*2^n)\neq \mathit{True})$}
%      \label{line:swmrma:writeSwap}
%         \State{$\mathit{val} \gets \mathit{R.read()}$}
%         \label{line:swmrma:writeRead}
%         % \State{$\mathit{new\_index} \gets \mathit{R_{index}.read()}$}
%         % \label{line:swmrma:writeRead}
%         % \State{$\mathit{new\_index} \gets \mathit{index} $}
%         \START[for] $0 \leq i < n$
%             \label{line:swmrma:loopAudit}
%                \START[if] $((\mathit{val} \pmod{2^{i+1}})/2^{i} = 1 \land p_i\not\in set)$
%              \Comment{$p_i$ read $\mathit{R}$ and is not in $\mathit{pairs}$}
%                 \label{line:swmrma:writecheckone}
%                 \State{$\mathit{pairs[index].write(p_i,val/2^n)}$}  
%                 \label{line:swmrma:writeAudit}
%                 \State{$set.add(p_i)$}  
%                 \label{line:swmrma:writeSet}
%                 \State{$\mathit{index} \gets \mathit{index} +1 $} 
%                 \label{line:swmrma:updateIndex}
%             \EndPhase
%         \EndPhase  
%         \State{$\mathit{R_{index}.write(index)}$}
%         \label{line:swmrma:writeIndex}
%     \EndPhase
%     % \State{$index \gets new\_index$}
%     \State{$set \gets \emptyset$}
%     \State{$val\gets v*2^n$}
%     \State{\textbf{return}}
% \EndPhase

% \end{algorithmic}
% }




{ % \footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Shared Variables:}
\Statex $\mathit{R}$: an object accessed by all processes, 
with \textit{read}, $compare\&swap$, and $fetch\&add$.
\Statex Holds an index (initially, $0$), a value (initially, $v_0$) and $n$ bits (all initially $0$)
\Statex $\mathit{pairs[\,]}$: 
an unbounded array of single-writer multi-reader registers (all initially $\perp$), 
written by the writer and read by all processes. 
\Statex 

\Statex \textbf{Local Variables:} \Comment{{\bf Pseudo code for reader and auditors $p_i$ ($i\in[0,n-1]$)}}
% \Statex $\mathit{temp}$ initially $\perp$ \Comment{store the content of the register}
\Statex $\mathit{read\_result}$ initially $\perp$ \Comment{the last value read}
\Statex $\mathit{temp}$ initially $\perp$ \Comment{the content of the register} 
% \Statex $\mathit{val}$ initially $\perp$ \Comment{value from S}
\Statex $\mathit{audit\_result}$ initially $\emptyset$ \Comment{set of (process, value) pairs} 
\Statex $\mathit{audit\_index}$ initially $0$ \Comment{index of the last updated value in pairs[]} 
\Statex $\mathit{last\_index}$ initially $0$ \Comment{index of the last audit operation} 
% \Statex $\mathit{int}$, initially $\perp$ \Comment{Information about $p_i$'s  read operation}

% \Statex

\START[Read()] 
    % \State{$index, \mathit{val} \gets \mathit{R.read()}$}
    \State{$temp \gets \mathit{R.read()}$}
    \label{line:swmrma:read}
    % \START[if]{ $(\mathit{val} \pmod{ 2^{(i+1)}})/2^{i} = 0$}
    \START[if]{ $(\mathsf{GetBits}(temp)[i] = 0)$}
    \label{line:swmrma:readCondition}
    % \State{$index,\mathit{read\_result},  \gets \mathit{R.fetch\&add}(2^i)$} 
    \State{$\mathit{read\_result}  \gets \mathsf{GetValue}(\mathit{R.fetch\&add}(2^i))$}
    % \State{$\mathit{read\_result}  \gets \mathsf{GetValue}(\mathit{R.fetch\&add}(WitnessValue(i)))$}
    \label{line:swmrma:readFetch}
    % \Comment{\textcolor{blue}{the fetch\&add exposes the structure}}
    \EndPhase
    \State{\textbf{return} $\mathit{read\_result}$}
    % \State{\textbf{return} $\mathit{read\_result}/2^n$}
    \label{line:swmrma:readReturn}
\EndPhase

\Statex

% \Statex \textbf{Local Variables:} \Comment{{\bf Pseudo code for auditor $p_j$}}
% \Statex $\mathit{val}$ initially $\perp$ \Comment{value from S}
% \Statex $\mathit{audit\_result}$ with initial value $\emptyset$ \Comment{set of the couples (process, value) of all the read operation} 
% \Statex $\mathit{audit\_index}$ with initial value $\emptyset$ \Comment{set of the couples (process, value) of all the read operation} 
% \Statex $\mathit{int}$, initially $\perp$ \Comment{\mathit{int}eger that stores information about $p_i$'s  last read operation}
\START[Audit()]
    % \State{$\mathit{audit\_index},\mathit{val} \gets \mathit{R.read()}$}
    \State{$\mathit{temp} \gets \mathit{R.read()}$}
    \label{line:swmrma:auditRead}
    \State{$\mathit{val} \gets \mathsf{GetValue}(temp)$}
    \State{$\mathit{audit\_index} \gets \mathsf{GetIndex}(temp)$}
    \START[for]{ $\mathit{last\_index} \leq j < \mathit{audit\_index}$}
        \State{$\mathit{audit\_result}.add(pairs[j].read())$}
        \label{line:swmrma:auditAddAuditPairs}
    \EndPhase
    \State{$\mathit{last\_index} \gets \mathit{audit\_index}$}
    \START[for] $0 \leq j < n$
        % \START[if] $(\mathit{val} \pmod{2^{i+1}})/2^{i} = 1$
        \START[if] $(\mathsf{GetBits}(temp)[j] = 1)$
            \Comment{checks if $p_j$ read the last value written in R}
            \label{line:swmrma:auditCondition}
            % \State{$\mathit{audit\_result}.add(p_i,\mathit{val}/2^{n})$}
            \State{$\mathit{audit\_result}.add(p_i,\mathit{val})$}
            \label{line:swmrma:auditAddAudit}
            % \State{$\mathit{last\_index} \gets \mathit{last\_index} +1$}
        \EndPhase
    \EndPhase  
        
    \State{\textbf{return} $\mathit{audit\_result}$}      
\EndPhase

\Statex

\Statex \textbf{Local Variables:} \Comment{{\bf  pseudo code for writer $p_0$}}
\Statex $\mathit{temp}$ initially $\perp$ \Comment{store the content of the register}
\Statex $\mathit{val}$ initially $v_0$ \Comment{the last value in the register}
\Statex $\mathit{index}$ initially $0$ \Comment{index of the last value in pairs[] } 
\Statex $\mathit{new\_index}$ initially $0$ \Comment{index of the last value in pairs[] } 
% \Statex $\mathit{int}$, initially $\perp$ \Comment{\mathit{int}eger coded with the $i+1$ low-order bits}

\START[Write($v$)]
    % \State{$\mathit{val} \gets v*2^{n}$}
    % \label{line:swmrma:writeHighOrder}
    % \Comment{Write $v$ in the high order bits}
    % \State{$\mathit{index},\mathit{val} \gets \mathit{R.read()}$}
    \State{$bits \gets 0^n$}
    \Comment{$0^n$ describe $n$ bits set to $0$}
    \START[while]{$(\mathit{R.compare\&swap}((\mathit{index},\mathit{val},bits),(\mathit{new\_index},v,0^n))\neq \mathit{True})$}
     \label{line:swmrma:writeSwap}
        % \State{$\mathit{index},\mathit{val} \gets \mathit{R.read()}$}
        \State{$\mathit{temp} \gets \mathit{R.read()}$}
        \label{line:swmrma:writeRead}
        % \State{$\mathit{new\_index} \gets \mathit{index} $}
        % \State{$\mathit prev_val \gets \mathsf{GetValue}(temp)$}
        \State{$\mathit bits \gets \mathsf{GetBits}(temp)$}
        \State{$\mathit{new\_index} \gets \mathsf{GetIndex}(temp) $}
        \START[for] $0 \leq j < n$
            \label{line:swmrma:loopAudit}
               % \State{$\mathit{\bit} \gets \mathit{val} \% 2^{i+1}$}  
            % \START[if] $(\mathit{val} \pmod{2^{i+1}})/2^{i} = 1$
            \START[if] $(bits[j] = 1)$
             \Comment{Checks if $p_j$ read the last value}
                \label{line:swmrma:writecheckone}
                % \State{$new\_pairs.add(p_i,\mathit{val})$}
                % \State{$\mathit{pairs[new\_index].write(p_i,val/2^n)}$}  
                \State{$\mathit{pairs[new\_index].write(p_j,val)}$} 
                \label{line:swmrma:writeAudit}
                \State{$\mathit{new\_index} \gets \mathit{new\_index} +1 $} 
                \label{line:swmrma:updateIndex}

            \EndPhase
        \EndPhase  
    \EndPhase
    \State{$index \gets new\_index$}
    \label{line:swmrma:updateNewIndex}
    \State{$val\gets v$}
    \State{\textbf{return}}
\EndPhase

\end{algorithmic}
}




















% { % \footnotesize
% \begin{algorithmic}[1]
% \Statex \textbf{Rhared Variables:}
% \Statex  $R$ Object shared between the $n$ processes that can be accessed through the following operations: \textit{read}, $compare\&swap$, $fetch\&add$. 


% \Statex

% \Statex \textbf{Local Variables:} \Comment{{\bf Pseudo code for reader $p_i$}}
% \Statex $\mathit{read\_result}$ with initial value $v_0$ \Comment{the last read value}
% \Statex $\mathit{val}$ with initial value $0$ \Comment{the timestamp of the last written value} 



% \Statex

% \START[Read()] 
%     \State{$\mathit{val} \gets S.read()$}
%     \START[if]{ $\lfloor(\\mathit{val}Mr \% 2^{(i+1)})/2^{i}\rfloor = 0$}
%     \State{$\mathit{read\_result},  \gets \mathit{R.fetch\&add}(2^i)$}
%     \EndPhase
%     \State{\textbf{return} \mathit{read\_result}}
% \EndPhase

% \Statex

% \Statex \textbf{Local Variables:} \Comment{{\bf Pseudo code for writer $p_0$}}
% \Statex $val$ with initial value $v_0$ written in the high order bits \Comment{the last read value}
% \Statex $index$ with initial value $\emptyset$ \Comment{the couple (process, value) of all the read operations} 
% \Statex $new\_pairs$ with initial value $\emptyset$ \Comment{the couple (process, value) of all the read operations} 
% \Statex $\mathit{int}$, initially $\perp$ \Comment{\mathit{int}eger coded with the $i+1$ low-order bits}

% \START[Write($v$)]
%     % \State{$val \gets v*2^{n}$}
%     % \label{line:swmrma:writeHighOrder}
%     % \Comment{Write $v$ in the high order bits}

%     \START[while]{$(S.compare\&swap((index,val),(\mathit{new\_index},v*2^n))\neq True)$}
%         \State{$index,val \gets S.read()$}
%         \State{$\mathit{new\_index} \gets index $}
%         \START[for] $0 \leq i < n$
%                \State{$\mathit{int} \gets val \% 2^{i+1}$}  
%                \START[if] $\lfloor \mathit{int}/2^{i}\rfloor = 1$
%              \Comment{Checks if $p_i$ read the last value}
%                 % \State{$new\_pairs.add(p_i,val)$}  
%                 \State{$pairs[index].write(p_i,val)$}  
%                 \State{$\mathit{new\_index} \gets \mathit{new\_index} +1 $}  

%             \EndPhase
%         \EndPhase  
%     \EndPhase
    
% \EndPhase

% \Statex

% \Statex \textbf{Local Variables:} \Comment{{\bf Pseudo code for auditor $p_j$}}
% \Statex $\mathit{val}$ initially $\perp$ \Comment{value from S}
% \Statex $\mathit{audit\_result}$ with initial value $\emptyset$ \Comment{set of the couples (process, value) of all the read operation} 
% \Statex $\mathit{int}$, initially $\perp$ \Comment{\mathit{int}eger that stores information about $p_i$'s  last read operation}
% \START[Audit()]
%     \State{$\mathit{audit\_result},val \gets S.read()$}
%     \START[for] $0 \leq i < n$
%                \State{$\mathit{int} \gets val \% 2^{i+1}$}  
%                \START[if] $\lfloor \mathit{int}/2^{i}\rfloor = 1$
%              \Comment{Checks if $p_i$ read the last value written in S}
%                 \State{$\mathit{audit\_result}.add(p_i,val)$}  
%             \EndPhase
%         \EndPhase  
%     \State{\textbf{return} \mathit{audit\_result}}      
% \EndPhase



% \end{algorithmic}
% }



% { % \footnotesize
% \begin{algorithmic}[1]
% \Statex \textbf{Rhared Variables:}
% \Statex  $R$ Object shared between the $n$ processes that can be accessed through the following operations: \textit{read}, $compare\&swap$, $fetch\&add$. 
% % \Statex  $Rseq_w$ Object shared between the writer and the readers that can be accessed through the following operations: \textit{read}, \textit{write}. 
% % \Statex $\forall i \in [1,n],\, Rseq_r[i]$ is an object shared between the readers that can be accessed through the following operations: \textit{read}, \textit{write}.

% \Statex

% \Statex \textbf{Local Variables:} \Comment{{\bf Pseudo code for reader $p_i$}}
% \Statex $\mathit{read\_result}$ with initial value $v_0$ \Comment{the last read value}
% \Statex $\mathit{val}$ with initial value $0$ \Comment{the timestamp of the last written value} 
% \Statex $seq$ with initial value $0$ \Comment{the timestamp of the last read value} 


% \Statex

% \START[Read()] 
%     \State{$\mathit{val} \gets max(Rseq_r[1-n].snapshot(),Rseq_w.read()$}
%     \START[if]{ $seq < \mathit{val}$}
%     \State{$seq, \mathit{read\_result},  \gets \mathit{R.fetch\&add}(2^i)$}
%     \State{$Rseq_r[i].write(seq)$}
%     % \State{$old\_ts=ts$}
%     \EndPhase
%     \State{\textbf{return} \mathit{read\_result}}
% \EndPhase

% \Statex

% \Statex \textbf{Local Variables:} \Comment{{\bf Pseudo code for writer $p_0$}}
% \Statex $val$ with initial value $v_0$ \Comment{the last read value}
% \Statex $seq$ with initial value $0$ \Comment{the timestamp of the last written value} 
% \Statex $pairs$ with initial value $0$ \Comment{the couple (pairs, value) of all the read operation} 

% \START[Write($v$)]      
%     \START[while]{$(S.compare\&swap((seq,val,pairs),(seq+1,v,pairs))\neq True)$}
%         \State{$seq,val,pairs \gets S.read()$}
%         % \State{$seq \gets seq + 1$}       
%     \EndPhase
%     \State{$seq \gets seq + 1$}  
%     \State{$Rseq\_w \gets seq$}
    
    
% \EndPhase

% \Statex

% \START[Audit()]
%     \State{$seq,val,pairs \gets S.read()$}
%     \State{\textbf{return} pairs}      
% \EndPhase



% \end{algorithmic}
% }


==> tables/Consensus_number.tex <==
\begin{table}
\centering
\caption{Consensus number of atomic register with audit operation}
\begin{tabular}{|l|l|l|l|l|}
\hline
Audit consistency & number of writers & number of readers & number of auditors & Consensus number  \\
\hline
Atomic & 1 & 1 & 1 & 2  \\
\hline
Atomic & 1 & n & 1 & 2  \\
\hline
Atomic & 1 & 1 & n & 2  \\
\hline
Atomic & 1 & n & n & n  \\
\hline
\hline
Regular & 1 & n & n & n \\
\hline
\end{tabular}
\end{table}
